Turbulence in Focus: Benchmarking Scaling Behavior of 3D Volumetric Super-Resolution with BLASTNet 2.0 Data

Analysis of compressible turbulent flows is essential for applications related to propulsion, energy generation, and the environment. Here, we present BLASTNet 2.0, a 2.2 TB network-of-datasets containing 744 full-domain samples from 34 high-fidelity direct numerical simulations, which addresses the current limited availability of 3D high-fidelity reacting and non-reacting compressible turbulent flow simulation data. With this data, we benchmark a total of 49 variations of five deep learning approaches for 3D super-resolution - which can be applied for improving scientific imaging, simulations, turbulence models, as well as in computer vision applications. We perform neural scaling analysis on these models to examine the performance of different machine learning (ML) approaches, including two scientific ML techniques. We demonstrate that (i) predictive performance can scale with model size and cost, (ii) architecture matters significantly, especially for smaller models, and (iii) the benefits of physics-based losses can persist with increasing model size. The outcomes of this benchmark study are anticipated to offer insights that can aid the design of 3D super-resolution models, especially for turbulence models, while this data is expected to foster ML methods for a broad range of flow physics applications. This data is publicly available with download links and browsing tools consolidated at https://blastnet.github.io.

==> diff_abs.tex <==
%DIF >  \doublespacing
\begin{abstract}
Analysis of compressible turbulent flows is essential for applications related to propulsion, energy generation, and the environment. 
Here, we present \textbf{BLASTNet 2.0}, a \textbf{2.2~TB} network-of-datasets containing \textbf{744 full-domain samples} from \textbf{34 high-fidelity direct numerical simulations}, which addresses the current limited availability of 3D high-fidelity reacting and non-reacting compressible turbulent flow simulation data.  With this data, we benchmark a total of \textbf{\DIFdelbegin \DIFdel{40 }\DIFdelend \DIFaddbegin \DIFadd{49 }\DIFaddend variations\DIFdelbegin %DIFDELCMD < \MBLOCKRIGHTBRACE %%%
\DIFdel{(with different model sizes) of three deep learning architectures }\DIFdelend \DIFaddbegin } \DIFadd{of five deep learning approaches }\DIFaddend for 3D super-resolution -- which can be applied for improving scientific imaging, simulations, turbulence models, as well as in computer vision  applications.
We perform neural scaling analysis on these models to examine the performance of different \DIFdelbegin \DIFdel{architectures, and to assess the benefits of a popular gradient-based physics-informed loss function across different model sizes}\DIFdelend \DIFaddbegin \DIFadd{machine learning (ML) approaches, including two scientific ML techniques}\DIFaddend . We demonstrate that (i) predictive performance \DIFdelbegin \DIFdel{(measured via structural-similarity image measure) }\DIFdelend can scale with model size and cost, (ii) \DIFdelbegin \DIFdel{the choice of }\DIFdelend architecture matters significantly, especially for smaller models, and (iii) the benefits of \DIFdelbegin \DIFdel{physics-informed }\DIFdelend \DIFaddbegin \DIFadd{physics-based }\DIFaddend losses can persist with increasing model size. The outcomes of this benchmark study are anticipated to offer insights that can aid the design of 3D super-resolution models, especially for turbulence models, while this data is expected to foster \DIFdelbegin \DIFdel{machine learning }\DIFdelend \DIFaddbegin \DIFadd{ML }\DIFaddend methods for a broad range of flow physics applications. This data is publicly available with download links and browsing tools consolidated at \url{https://blastnet.github.io}.
\end{abstract}

==> diff_content.tex <==
\DIFdelbegin %DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdelend %DIF >  \doublespacing
\section{Introduction}
\setcounter{footnote}{0} 
In recent years, machine learning (ML) has offered new modeling approaches for natural and engineering sciences. 
% For example, a 25TB open-source dataset~\cite{varadi_alphafolddata} (with 214M protein samples) enabled AlphaFold 2~\cite{Jumper2021} to achieve breakthrough predictive accuracy in the difficult challenge of protein-folding prediction. 
For example, 5~PB of ERA5 data~\cite{hersbach} was employed towards GraphCast~\cite{lam2022graphcast}, an ML model that outperformed conventional weather modeling techniques. 
As such, efforts in \DIFdelbegin \DIFdel{building and }\DIFdelend curating large datasets for scientific ML \DIFdelbegin \DIFdel{applications }\DIFdelend have been growing across numerous domains including agricultural science~\cite{kondmanDenethor}, geophysics~\cite{deng2022openfwi}, and biology~\cite{varadi_alphafolddata}. In many of these examples, the volume of data  can significantly exceed the free limit of open-source repositories such as \DIFdelbegin \DIFdel{Zenodo (50~GB) and }\DIFdelend Kaggle (100~GB) -- typically used to store and share language and image data -- due to potentially high dimensions within scientific data. As such, significant resources are required for building and maintaining  data storage \DIFdelbegin \DIFdel{facilities}\DIFdelend \DIFaddbegin \DIFadd{capabilities}\DIFaddend , either through institutional collaborations~\cite{kondmanDenethor,varadi_alphafolddata,TAGHIZADEHPOPP2020100412} or cloud service providers~\cite{cloud}. 

\DIFdelbegin %DIFDELCMD < \begin{wrapfigure}[18]{r}{0.405\textwidth}    \centering
%DIFDELCMD < \vspace{-5mm}
%DIFDELCMD < \includegraphics[width=0.405\textwidth]{figs/dataset_summary.pdf}
%DIFDELCMD <   %%%
%DIF <  \caption{Collection and distribution strategy for TB-scale data. \label{fig:collect}}
  %DIF <  \vspace{-5mm}
%DIFDELCMD < \caption{%
{%DIFAUXCMD
\DIFdel{Datasets used for this study. }%DIFDELCMD < \label{fig:blastnet_data}%%%
}
%DIFAUXCMD
%DIFDELCMD < \end{wrapfigure}
%DIFDELCMD < %%%
\DIFdelend In previous work~\cite{chung2022the,chung2022aecs}, we proposed the Bearable Large Accessible Scientific Training Network-of-datasets (BLASTNet), a cost-effective community-driven weakly centralized framework (see \Cref{sec:blastnet_data}) for increasing access to \DIFdelbegin \DIFdel{high-dimensional scientific data.
With this, we }\DIFdelend \DIFaddbegin \DIFadd{scientific data, which }\DIFaddend provided access to 110 full-domain samples from 10 configurations (225~GB) of 3D high-fidelity flow physics \DIFdelbegin \DIFdel{simulations}\DIFdelend \DIFaddbegin \DIFadd{direct numerical simulations (DNS)}\DIFaddend . 
In this work, we present the updated {BLASTNet 2.0 dataset}, which is extended to{ 744 full-domain samples from 34 \DIFaddbegin \DIFadd{DNS }\DIFaddend configurations, as shown in \Cref{fig:blastnet_data}. This dataset aims to address \DIFdelbegin \DIFdel{(i) }\DIFdelend limitations in data availability for compressible turbulent non-reacting and reacting  flows, which \DIFdelbegin \DIFdel{have a wide range of applications }\DIFdelend \DIFaddbegin \DIFadd{is found }\DIFaddend in automotive~\cite{chungijer,guo2023analysis}, propulsion~\cite{bitter2011high,hickey2013large}, energy~\cite{temme2014combustion,esclapez2017fuel}, and environmental\DIFdelbegin \DIFdel{problems~\mbox{%DIFAUXCMD
\cite{mueller2014large,morandini2018fire} }\hskip0pt%DIFAUXCMD
.  }\DIFdelend \DIFaddbegin \DIFadd{~\mbox{%DIFAUXCMD
\cite{mueller2014large,morandini2018fire} }\hskip0pt%DIFAUXCMD
applications.  
}

\DIFaddend From BLASTNet 2.0, we \DIFdelbegin \DIFdel{extract }\DIFdelend \DIFaddbegin \DIFadd{pre-process DNS  data to form }\DIFaddend the {Momentum128 3D SR dataset} for benchmarking models aimed at 3D super-resolution (SR) of turbulent flows. 
%DIF <  Our benchmark focuses on investigating the cost and predictive performance of three different model architecture approaches, along with their scaling properties. We choose this task due to its wide range of uses across different flow physics applications~\cite{peterson2013high,guo2023analysis,bitter2011high,hickey2013large,temme2014combustion,esclapez2017fuel,mueller2014large,morandini2018fire,ravela2010realtime,de2020turbulent}, and its broader applicability to 3D SR problems in media~\cite{nah2019ntire} and other scientific domains~\cite{liu2021dl,Xue22}.
%DIF >  SR is an ML task that has broad applicability within domains tied to computer vision, scientific and medical imaging, as well as flow physics.
To this end,  we:
\begin{itemize}
    \item Curate BLASTNet 2.0, a diverse public 3D compressible turbulent flow \DIFaddbegin \DIFadd{DNS }\DIFaddend dataset.
    \item Benchmark performance and cost of \DIFaddbegin \DIFadd{five }\DIFaddend 3D \DIFdelbegin \DIFdel{versions of  three popular SR models~\mbox{%DIFAUXCMD
\cite{wang2018esrgan,lim2017enhanced,zhang2018image} }\hskip0pt%DIFAUXCMD
}\DIFdelend \DIFaddbegin \DIFadd{ML approaches~\mbox{%DIFAUXCMD
\cite{wang2018esrgan,lim2017enhanced,zhang2018image,yu2022gradient,WEN2022104180} }\hskip0pt%DIFAUXCMD
for  SR  }\DIFaddend with this publicly accessible dataset.
    \item Show that SR model performance can
scale with the logarithm of model size and cost.
    \item Demonstrate the persisting benefits of a popular gradient-based \DIFdelbegin \DIFdel{physics-informed }\DIFdelend \DIFaddbegin \DIFadd{physics-based }\DIFaddend loss~\cite{yu2022gradient} with increasing model size.
\end{itemize}

\begin{figure}   \centering
\includegraphics[width=0.405\textwidth]{figs/dataset_summary.pdf}
  %DIF >  \caption{Collection and distribution strategy for TB-scale data. \label{fig:collect}}
  %DIF >  \vspace{-5mm}
\caption{{Datasets used for this study. }\label{fig:blastnet_data}}
\end{figure}
\DIFdelbegin \DIFdel{We provide a brief }\DIFdelend  
 \DIFadd{We provide an }overview of related efforts in \DIFdelbegin \DIFdel{turbulent SR, public-access flow physics datasets, and SR benchmarks in }\DIFdelend \Cref{sec:related}. In \Cref{sec:data}, we provide information on the BLASTNet 2.0 and Momentum128 3D SR datasets.  Our benchmark setup is described in \Cref{sec:method}, \DIFdelbegin \DIFdel{while our results are }\DIFdelend \DIFaddbegin \DIFadd{with results }\DIFaddend discussed in \Cref{sec:results}, before \DIFdelbegin \DIFdel{presenting concluding remarks }\DIFdelend \DIFaddbegin \DIFadd{the conclusions }\DIFaddend in \Cref{sec:conc}.

\section{Related Work}
\label{sec:related}
  % Coarse-graining and averaging removes information about turbulence. 

% \textbf{ML for Turbulence Modeling} 
  % The governing equations for fluid systems are well-known. Thus, solving the Navier-Stokes equations and related conservation equations with numerical solvers can provide high-fidelity information, as long the simulation grid resolves the Kolmogorov lengthscale~\cite{pope2000turbulent} -- the smallest eddies within continuum flows. These direct numerical simulations (DNS) involve billions of voxels and months of computation on supercomputing facilities~\cite{find}. Due to these significant computational costs, DNS is restricted for investigating fundamental flow behavior and is not widely applicable to practical flows in engineering systems (engines, rockets, climate, wildfires, \textit{etc.}).
  % Thus, it is common to reduce the resolution by computing on coarser grids with large eddy simulations (LES), or by evolving time-/ensemble- averaged quantities   with Reynolds-averaged Navier-Stokes (RANS) simulations. Coarse-graining and averaging removes information about turbulence. This information is typically recovered through  \textit{closure modeling}~\cite{pope2000turbulent,vreman2004,colin2000thickened}, which has been subject to numerous ML studies involving tabular ML~\cite{CHUNG202211175,find} and deep learning models~\cite{lapeyre2019training,find}. \comment{add physics informed loss as a topic}. \comment{mention that benchmark studies are not widely performed due to data access. thus your work is novel}

\paragraph{Flow Physics Simulation Datasets} \DIFdelbegin \DIFdel{The governing equations for flow physicsare well-known for a wide range of conditions. Thus, numerical simulations can provide high-fidelity information, }\DIFdelend \DIFaddbegin \DIFadd{Numerical simulations accurately describe flow physics, }\DIFaddend as long as the simulation grid resolves the smallest lengthscales associated with turbulent dissipation~\cite{pope2000turbulent}. \DIFdelbegin \DIFdel{A high-fidelity direct numerical simulation (DNS) can involve  }\DIFdelend \DIFaddbegin \DIFadd{With up to }\DIFaddend $\mathcal{O}(10^9)$ voxels, $\mathcal{O}(10^6)$ \DIFdelbegin \DIFdel{CPU-hours }\DIFdelend \DIFaddbegin \DIFadd{core-hours }\DIFaddend of simulation time, and $\mathcal{O}(10^4)$ \DIFdelbegin \DIFdel{CPUs }\DIFdelend \DIFaddbegin \DIFadd{computer cores }\DIFaddend on parallel computing facilities~\DIFdelbegin \DIFdel{\mbox{%DIFAUXCMD
\cite{JUNG2021111584,JIANG2021111432,brouzet_talei_brear_cuenot_2021}}\hskip0pt%DIFAUXCMD
. 
Due to these significant computational costs, DNS is not applicable to }\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\cite{JUNG2021111584,JIANG2021111432,brouzet_talei_brear_cuenot_2021,WANG2022108292}}\hskip0pt%DIFAUXCMD
, high-fidelity DNS of }\DIFaddend many real-world flows \DIFdelbegin \DIFdel{without careful consideration}\DIFdelend \DIFaddbegin \DIFadd{cannot be performed due to prohibitive costs}\DIFaddend .
  Thus, it is common to employ coarser grids with large-eddy simulations (LES)~\cite{esclapez2017fuel,huang2020}, or by only evolving  time-/ensemble-averaged quantities with Reynolds-averaged Navier-Stokes (RANS) simulations~\cite{mcconkey2021curated,bonnet2022airfrans} -- both of which rely on turbulence models that can be discovered from DNS data. DNS data is also useful for  applications involving  scientific imaging~\cite{Gunes2007}, spatio-temporal modeling~\cite{stachenfeld2022learned}, and solving inverse problems~\cite{raissi_inverse}. As shown \DIFaddbegin \DIFadd{in }\DIFaddend \Cref{tab:datasets}, many existing flow simulation datasets focus on LES and RANS simulations due to data storage constraints. 
  % However, flows exist in a wide range of conditions that available datasets cannot address. For example,~
  \citet{mcconkey2021curated} recently released a dataset for improving  turbulence models in incompressible  \DIFdelbegin \footnote{\DIFdel{Pressure in incompressible flow is treated with an elliptic PDE. In high Mach number compressible flows, pressure is treated with a state equation, resulting in PDE behavior that can form discontinuities (shocks).}}  %DIFAUXCMD
\addtocounter{footnote}{-1}%DIFAUXCMD
\DIFdelend non-reacting RANS. 
 AirfRANS~\cite{bonnet2022airfrans} provides both 2D incompressible and compressible non-reacting RANS data, specifically on airfoil configurations. For reacting flows,~\citet{huang2020} released a 2D LES dataset for developing reduced-order models. 
 \DIFdelbegin \DIFdel{We note that 2D flow simulations are typically not representative of a wide range of flow systems due to limitations in treating vortex stretching~\mbox{%DIFAUXCMD
\cite{pope2000turbulent}}\hskip0pt%DIFAUXCMD
. 
 }\DIFdelend The largest flow physics dataset, the Johns Hopkins Turbulence Database (JHTDB)~\cite{Yi2008}, provides 3D DNS data from turbulent incompressible non-reacting flow simulations. 
 Since these datasets are either 2D, incompressible, or non-reacting, they are not suitable for many applications involving aerodynamics, propulsion, or chemical processes\DIFaddbegin \footnote{\DIFadd{Pressure in incompressible flows is typically treated with an elliptic partial differential equation (PDE). In high Mach number compressible flows, pressure is treated with a state equation, resulting in PDE behavior that can form discontinuities (shocks). 2D flow simulations are typically not representative of a wide range of flow systems due to limitations in treating vortex stretching~\mbox{%DIFAUXCMD
\cite{pope2000turbulent}}\hskip0pt%DIFAUXCMD
}}\DIFaddend . This is one reason why 
 ML studies involving these applications employ self-generated inaccessible datasets~\cite{BODE20212617,ihme2022combustion} -- introducing challenges to \DIFdelbegin \DIFdel{fair/}\DIFdelend open model evaluation.   
 To address these gaps,  we curate BLASTNet 2.0, a 3D turbulent compressible reacting and non-reacting flow dataset, which targets a balance of diversity, fidelity, and size.

\begin{table}[htb]
\DIFdelbeginFL %DIFDELCMD < \vspace{-2.5mm}
%DIFDELCMD < \fontsize{8.7pt}{8.7pt}%%%
\DIFdelendFL \DIFaddbeginFL \vspace{-3.5mm}
\fontsize{8pt}{8pt}\DIFaddendFL \selectfont
\setlength{\tabcolsep}{2.3mm} % General space between cols (6pt standard)
\renewcommand{\arraystretch}{1.3} % General space between rows (1 standard)
\begin{center}
\caption{Comparison of BLASTNet 2.0 (in \textbf{bold}) with selected flow simulation datasets.\label{tab:datasets}}
\vspace{11pt}
\begin{tabular}{lcccccc}

\toprule 
\multirow{2}{*}{Datasets}                          & \multicolumn{2}{c}{\textbf{BLASTNet}}                                                                                                                                         & \multirow{2}{*}{JHTDB~\cite{Yi2008}}                                                                         &  McConkey  & \multirow{2}{*}{AirfRANs~\cite{bonnet2022airfrans}}                                                          & \multirow{2}{*}{\citet{huang2020}}     \\
\cline{2-3}

& \textbf{2.0} &  
 1.0~\cite{chung2022aecs}&  &et al.~{\cite{mcconkey2021curated}} &\\
\midrule 
Size {[}TB{]}             & \textbf{{2.2} }                                                           & {0.225}                                                          & {490}    &{0.014}                          & {0.066}                                          & {0.209}                                                                                             \\
 Configs.            &\textbf{{34}}                                                             & {10}                                                              & {10}                    & 29                             & 1,000                                           & {1}                                                                                            \\
 Full-domain Samples & \textbf{744} & 120 & 15,791 & 29 & 1,000 &   30,000 \\
\midrule
Fidelity                  & \multicolumn{2}{c}{\textbf{DNS}}                                                                                                                                          &        DNS       & RANS                                               & RANS                                                           &               LES                                                                                                       \\
% Next-frame?            & \multicolumn{2}{c|}{\textbf{Partial}}                                                                                 & Partial         & No                                                 & No                                                                 & Yes                                                                                                                   \\
Spatial Dimensions        & \multicolumn{2}{c}{\textbf{3D}}                                                                           &                                                        3D              & 2D,3D                                              & 2D                                                                 & 2D                                                \\
Primitive Variables\tablefootnote{Filtered and time-/ensemble-averaged quantity $\phi$ is expressed with $\ol{\phi}$ and $\langle \phi \rangle$, respectively. In compressible LES, Favre-filtering $\widetilde{\phi}$~\cite{peters_2000} is typically used. $T$ refers to temperature; more definitions in \Cref{eq:dns}.} & 
\multicolumn{2}{c}{$\boldsymbol{u_i}$,$\boldsymbol{p}$,$\boldsymbol{T}$,$\boldsymbol{\rho}$,$\boldsymbol{Y_k}$}
& $u_i$,$p$,$\rho$,\DIFdelbeginFL \DIFdelFL{$b$                                      }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{$b_i$                                      }\DIFaddendFL & $\langle u_i\rangle$,$\langle p\rangle$                                            & $\langle u\rangle_i$,$\langle p\rangle$,$\langle T\rangle$,$\langle\rho\rangle$     &     $\widetilde{u}_i$,$\ol{p}$,$\widetilde{T}$,$\ol{\rho}$,$\widetilde{Y}_k$    \\
Number of PDEs\DIFaddbeginFL \tablefootnote{PDEs for continuity, energy, momentum, chemical species, and magnetic field $b_i$.} \DIFaddendFL & \multicolumn{2}{c}{\textbf{5 to 27}} & 4 to \DIFdelbeginFL \DIFdelFL{5 }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{7 }\DIFaddendFL & 3 to 4 & 4 to 5 & 7
\\Compressible Flow? & \multicolumn{2}{c}{{\textbf{Yes}}} & {No}& {No} & Yes\tablefootnote{This dataset contains a blend of compressible and incompressible flow samples.} & {Yes}\\ 
Multi-physics? & \multicolumn{2}{c}{{\textbf{Reactions}\tablefootnote{Majority are reacting flows. Some non-reacting flows are present.}}}  & {MHD\tablefootnote{Only one of the ten configurations consider magneto-hydrodynamics (MHD).}} & {No }& {No} & {Reactions}\\
\midrule
Host                      & \multicolumn{2}{c}{\textbf{Kaggle}}                                                                                                                                                        & SciServer~\cite{TAGHIZADEHPOPP2020100412}     & Kaggle                                             & Sorbonne &  UMich           \\                Format  & \multicolumn{2}{c}{\textbf{ \lstinline{.dat} }} &\lstinline|.h5|&\lstinline|.npy|&        \lstinline|.vtu|,\lstinline|.vtp|               & \lstinline|ascii|         \\
\bottomrule 
\end{tabular}
\end{center}
% \vspace{-7mm}
\vspace{-4mm}
\end{table}


\paragraph{SR for Turbulent Flows} 
\DIFdelbegin \DIFdel{High-fidelity (but costly) experimental measurements and simulations have been essential for understanding turbulent flows in a wide range of natural and engineering systems~\mbox{%DIFAUXCMD
\cite{chungijer,guo2023analysis,bitter2011high,hickey2013large,temme2014combustion,esclapez2017fuel,mueller2014large,morandini2018fire,ravela2010realtime,de2020turbulent}}\hskip0pt%DIFAUXCMD
. As such}\DIFdelend %DIF >  High-fidelity (but costly) experimental measurements and simulations have been essential for understanding turbulent flows in a wide range of natural and engineering systems~\cite{chungijer,guo2023analysis,bitter2011high,hickey2013large,temme2014combustion,esclapez2017fuel,mueller2014large,morandini2018fire,ravela2010realtime,de2020turbulent}. 
\DIFaddbegin \DIFadd{Within experimental flow measurements}\DIFaddend ,  deep learning-based SR approaches \DIFdelbegin \DIFdel{for turbulent flows have been gaining popularity in both experiments~\mbox{%DIFAUXCMD
\cite{zhiwen_phys,wang2022deep} }\hskip0pt%DIFAUXCMD
and simulation~\mbox{%DIFAUXCMD
\cite{BODE20212617,fukami2019super,linqi}}\hskip0pt%DIFAUXCMD
. 
Within flow simulations , }\DIFdelend \DIFaddbegin \DIFadd{have been employed towards improving Schlieren~\mbox{%DIFAUXCMD
\cite{wang2020deep}}\hskip0pt%DIFAUXCMD
, particle-image-velocimetry~\mbox{%DIFAUXCMD
\cite{zhiwen_phys}}\hskip0pt%DIFAUXCMD
, and tomography~\mbox{%DIFAUXCMD
\cite{janssens2020computed} }\hskip0pt%DIFAUXCMD
techniques, which can often be limited by resolution restrictions. 
In many practical engineering analyses, coarse-grained simulations with under-resolved grid sizes are often used to bypass the extensive costs of fully-resolved DNS. A dominant source of error from this approach involves missing physics that arise from the under-resolved grid, as will be detailed in }\Cref{sec:metrics}\DIFadd{. While algebraic turbulence models have been traditionally used to represent the under-resolved physics~\mbox{%DIFAUXCMD
\cite{germano1991dynamic,vreman2004}}\hskip0pt%DIFAUXCMD
, specific algebraic models are effective only in specific flow configurations~\mbox{%DIFAUXCMD
\cite{moser2021statistical}}\hskip0pt%DIFAUXCMD
. }\DIFaddend SR and related upsampling approaches have been proposed \DIFaddbegin \DIFadd{as a versatile alternative }\DIFaddend for correcting under-resolved information from coarse-grid simulations between numerical time-stepping~\DIFdelbegin \DIFdel{\mbox{%DIFAUXCMD
\cite{BODE20212617}}\hskip0pt%DIFAUXCMD
}\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\cite{BODE20212617,fukami2019super,linqi}}\hskip0pt%DIFAUXCMD
}\DIFaddend , which would require considerations of real-time inferencing. Studies on turbulent SR have focused \DIFdelbegin \DIFdel{primarily }\DIFdelend on demonstrating feasibility~\DIFdelbegin \DIFdel{\mbox{%DIFAUXCMD
\cite{BODE20212617,zhiwen_phys,wang2022deep,fukami2019super,linqi}}\hskip0pt%DIFAUXCMD
}\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\cite{BODE20212617,zhiwen_phys,fukami2019super,linqi,wang2022deep}}\hskip0pt%DIFAUXCMD
}\DIFaddend , mostly by modifying existing image SR models. Due to memory constraints, many of these studies focus on 2D configurations~\DIFdelbegin \DIFdel{\mbox{%DIFAUXCMD
\cite{zhiwen_phys,wang2022deep,fukami2019super} }\hskip0pt%DIFAUXCMD
(which are not applicable to many real-world flows)}\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\cite{zhiwen_phys,fukami2019super,wang2022deep}}\hskip0pt%DIFAUXCMD
}\DIFaddend , with 3D SR investigations only demonstrated recently~\cite{BODE20212617,linqi}. 
As such, there has not yet been a detailed and reproducible benchmark study comparing \DIFdelbegin \DIFdel{the performance and cost of }\DIFdelend SR models for 3D turbulent flows~\cite{ihme2022combustion,sharma}.

\DIFaddbegin \paragraph{\DIFadd{Scientific ML Approaches}} \DIFadd{Scientific ML approaches can involve developing custom architectures with implicit biases that suit specific problems and  modifying loss functions with constraints related to governing equations~\mbox{%DIFAUXCMD
\cite{Karniadakis2021}}\hskip0pt%DIFAUXCMD
. 
Firstly, model architectures such as  NUNet~\mbox{%DIFAUXCMD
\cite{obiolssales2022nunet}}\hskip0pt%DIFAUXCMD
, MeshGraphNet~\mbox{%DIFAUXCMD
\cite{pfaff2021learning}}\hskip0pt%DIFAUXCMD
, and Fourier Neural Operators (FNO)~\mbox{%DIFAUXCMD
\cite{li2021fourier} }\hskip0pt%DIFAUXCMD
employ graph and spectral convolution layers to ensure that flow predictions are mesh invariant. While FNOs have been successfully employed towards canonical laminar flow configurations, previous studies have demonstrated that these models are insufficiently expressive for complex configurations, involving turbulent~\mbox{%DIFAUXCMD
\cite{stachenfeld2022learned} }\hskip0pt%DIFAUXCMD
and  multi-physics~\mbox{%DIFAUXCMD
\cite{WEN2022104180} }\hskip0pt%DIFAUXCMD
flows. This has been attributed to regularization properties of spectral convolution layers by the FNO's original developers~\mbox{%DIFAUXCMD
\cite{WEN2022104180}}\hskip0pt%DIFAUXCMD
.
Recently, convolution FNO (Conv-FNO)~\mbox{%DIFAUXCMD
\cite{WEN2022104180} }\hskip0pt%DIFAUXCMD
models have been proposed to ameliorate these underfitting issues by embedding convolutional blocks within FNO blocks. Secondly, modifying the loss functions can involve adding a regularization term based on the residuals of the entire governing equations~\mbox{%DIFAUXCMD
\cite{RAISSI2019686}}\hskip0pt%DIFAUXCMD
. A softer approach involves regularizing with individual operators within the governing equation (such as continuity, advection, diffusion, and source terms)~\mbox{%DIFAUXCMD
\cite{BODE20212617}}\hskip0pt%DIFAUXCMD
. 
In this work, we benchmark models based on both loss function and architecture approaches, }\textit{\DIFadd{i.e.}}\DIFadd{, a model with a gradient-based loss function~\mbox{%DIFAUXCMD
\cite{yu2022gradient} }\hskip0pt%DIFAUXCMD
(which biases ML optimization towards turbulence applications; see }\customref{sec:loss}\DIFadd{) and a Conv-FNO model, respectively.
}


\DIFaddend \paragraph{SR Benchmarks}  SR via deep learning has been subjected to numerous competition and benchmark studies targeting various aspects of 2D image SR, including 2K-images~\cite{Agustsson_2017_CVPR_Workshops}, night photography~\cite{Ershov_2022_CVPR}, spectral recovery~\cite{Arad_2022_CVPR}, and satellite images~\cite{cornebise2022open}. For 3D SR, benchmarks for video~\cite{nah2019ntire}, medical resonance imaging~\cite{liu2021dl}, and 3D microscopy applications~\cite{Xue22} have been performed. Another method for studying the behavior of deep learning models involves the construction of empirical scaling relationships~\cite{hoffmann2022an}. This type of analysis has been useful for studying resource requirements of large language models, and was briefly been employed for studying 2D SR with a U-Net model~\cite{klug2023scaling}. Given the potential real-time computing applications of turbulent SR,  this analysis provides useful information on the relationship between model size, cost, and predictive performance. 
%To our knowledge, 3D SR benchmarks and scaling law analysis for turbulent flow applications have not been explore extensively prior to this work.




\section{Dataset}
\label{sec:data}
% This work highlights the release of (i) the BLASTNet 2.0 dataset, and (ii) the Momentum128 3D SR dataset extracted from BLASTNet 2.0, as summarized in \Cref{fig:blastnet_data}.



\subsection{BLASTNet 2.0}
\label{sec:blastnet_data}

 BLASTNet 2.0 consists of turbulent compressible flow DNS data\DIFaddbegin \DIFadd{, }\DIFaddend on Cartesian spatial grids\DIFdelbegin \DIFdel{. All data is }\DIFdelend \DIFaddbegin \DIFadd{, }\DIFaddend generated by solving \DIFdelbegin \DIFdel{the }\DIFdelend governing equations for mass, momentum, \DIFdelbegin \DIFdel{total }\DIFdelend energy, and chemical species, respectively: 
\begin{subequations}\label{eq:dns}
\begin{align}
    \partial_t {\rho} + \nabla \cdot ({\rho} {\mathbf{u}} ) &= 0~, \label{eq:continuity} \\
    %%%%%% eq2
    \partial_t ({\rho} {\mathbf{u}}) + \nabla \cdot ({\rho} {\mathbf{u}} \otimes{\mathbf{u}} ) &= 
    - \nabla p
      + \nabla \cdot {\boldsymbol{\tau}}~, \label{eq:momentum}\\ 
    %%%%% eq3
    \partial_t ({\rho} {e^t}) + \nabla \cdot [{\mathbf{u}} ({\rho}  {e^t} + {p})] &=  - \nabla \cdot {\mathbf{q}} +
    \nabla \cdot [ 
    ({\boldsymbol{\tau}}  )\cdot {\mathbf{u}}]~, \DIFaddbegin \label{eq:energy_conserve}
    \DIFaddend \\
%%%%%%
    \partial_t ({\rho} Y_k) + \nabla \cdot ({\rho} {\mathbf{u}} Y_k) &= 
    -\nabla \cdot \mathbf{{j}}_k + {\dot{\omega}}_k\, ,
\end{align}
\end{subequations}
with density $\rho$, velocity vector $\mathbf{u}$, pressure $p$,  specific total energy $e^t$, stress tensor $\boldsymbol{\tau}$, and  heat flux $\mathbf{q}$. $Y_k$, $\mathbf{j}_k$, and $ {\dot{\omega}_k}$ are the mass fraction, diffusion flux, and source term for chemical species $k~=~[1,N_s-1]$, where $N_s$ is the number of species. Molecular fluxes are typically modeled using the
mixture-averaged diffusion model. 
% The governing equations are closed by an equation of state (ideal gas or Peng-Robinson~\cite{preos}). %Note that \Cref{eq:continuity,eq:momentum} represent the compressible Navier-Stokes equations, which require a different numerical treatment from the incompressible Navier-Stokes equations, as detailed in the Supplementary Material.
This dataset is developed with these properties in mind:

\paragraph{Fidelity} All DNS data is collected  from well-established numerical solvers~\cite{brouzet_talei_brear_cuenot_2021,MA2017330,Chen_2009,DESJARDINS20087125,POLUDNENKO2010995} \DIFdelbegin \DIFdel{having }\DIFdelend \DIFaddbegin \DIFadd{with }\DIFaddend spatial discretization schemes ranging from 2nd- to 8th-order accuracy, while time advancement accuracy range from 2nd- to 4th-order.  \DIFdelbegin \DIFdel{All }\DIFdelend \DIFaddbegin \DIFadd{Low-order schemes require finer discretizations compared to high-order schemes, to achieve similar accuracy and numerical stability~\mbox{%DIFAUXCMD
\cite{moin1998}}\hskip0pt%DIFAUXCMD
. However, all }\DIFaddend simulations are spatially resolved to the order of the Kolmogorov lengthscale, ranging from 3.9 to 41 $\mu$m depending on the configuration\DIFaddbegin \DIFadd{, with a corresponding temporal discretization that ensures numerical stability}\DIFaddend . 

\paragraph{Size and Diversity} 
%As discussed in \Cref{sec:related}, turbulent flow data can become impractically large without careful consideration.  
BLASTNet 2.0 contains a total of 744 full-domain samples (2.2~TB) from a diverse collection of 34 simulation configurations: non-reacting decaying homogeneous isotropic turbulence (HIT)~\cite{CHUNG2022111758}, reacting forced HIT~\cite{POLUDNENKO2010995}, two parametric variations of reacting jet flows~\cite{brouzet_talei_brear_cuenot_2021}, six configurations of non-reacting transcritical channel flow~\cite{guo_yang_ihme_2022}, a reacting channel flow~\cite{JIANG2021111432}, a partially-premixed slot burner configuration~\cite{JUNG2021111584}, and 22 parametric variations (with different turbulent and chemical timescales) of a freely-propagating flame configuration~\cite{SAVARD2019402}.

\paragraph{Community-involvement} BLASTNet 2.0 consists of data contributions from six different institutions. As mentioned in \customref{sec:maintain}, our long-term vision and maintenance plan for this dataset involves seeking additional contributions from members of the broader flow community. 

\paragraph{Cost-effective Storage, Distribution, and Browsing} To circumvent Kaggle storage constraints, we partition the data into a network of $<100$~GB subsets, with each subset containing  a separate simulation configuration. This partitioned data can then be uploaded as separate datasets on Kaggle. To consolidate access to this data, all Kaggle download links are presented in \url{https://blastnet.github.io}, with the inclusion of a \lstinline{bash} script for downloading all \DIFdelbegin \DIFdel{the }\DIFdelend data through the Kaggle API. In addition, Kaggle notebooks are attached to each subset to enable convenient data browsing on Kaggle's cloud computing platform. This approach enables cost-effective distribution of scientific data that adheres to FAIR principles~\cite{Wilkinson2016}, as further detailed in \customref{sec:maintain}.

\paragraph{Consistent Format} Data, generated from different numerical solvers, initially exists  in a range of formats (\lstinline{.vtk}, \lstinline{.vtu}, \lstinline{.tec}, and \lstinline{.dat}) that are not readily formatted for training ML models. Thus, all flowfield data are processed into a consistent format -- little-endian single-precision binaries that can be read with \lstinline{np.fromfile}/\lstinline{np.memmap}. The choice of this data format enables high I/O speed in loading arrays. We  provide \lstinline{.json} files that store additional information on configurations, chemical mechanisms and transport properties. \DIFdelbegin \DIFdel{More information is provided in }\DIFdelend \DIFaddbegin \DIFadd{See }\DIFaddend \customref{sec:dataformat} \DIFaddbegin \DIFadd{for more details}\DIFaddend . 

\paragraph{Licensing and Ethics}  All data is generated by the present authors and licensed via  CC~BY-NC-SA~4.0. Other than the contributors' names and institutions, no personal-identifiable information is published in this data. No offensive content is published with this flow physics dataset. Further discussion on negative impact is provided in \Cref{sec:conc}.




% \begin{figure}
%     \centering
%     \begin{minipage}{.67\textwidth}
% \centering
% \includegraphics[width=\textwidth]{figs/collect_dist.pdf}
%   \caption{Collection and distribution strategy for TB-scale data. \label{fig:collect}}
% \end{minipage}
% \begin{minipage}{.32\textwidth}
%     \centering
% \includegraphics[width=\textwidth]{figs/distill.pdf}
%     \caption{Distilling BLASTNet 2.0 into the present dataset.}
%     \label{fig:distill}
% \end{minipage}
% \end{figure}



\subsection{Momentum128 3D SR Dataset}
\label{sec:mom_data}
BLASTNet 2.0 \DIFdelbegin \DIFdel{should be further processed before }\DIFdelend \DIFaddbegin \DIFadd{is further processed for }\DIFaddend training due to constraints in (i) memory and (ii) grid properties. \DIFdelbegin \DIFdel{For instance}\DIFdelend \DIFaddbegin \DIFadd{Currently}\DIFaddend , the single largest sample (92 GB) in BLASTNet 2.0 contains 1.3B voxels and 15 channels, which cannot fit into typical GPU memory. In addition, the spatial grid is stretched depending on the resolution requirements of the flow domain. As shown in \Cref{fig:blastnet_data}, we circumvent these two issues by sampling $128^3$ sub-volumes of density $\rho$ and velocity $\mathbf{u}$ from the uniform regions from all BLASTNet data. This results in 12,750 sub-volume samples (427~GB). We choose this sub-volume size to enable 32$\times$~SR (the resulting feature sub-volume is $4^3$ which is larger than a kernel size of 3), while maintaining a low memory footprint. In order to develop a compressible turbulence benchmark dataset that can be easily downloaded, we select 2,000 sub-volumes to form a 67~GB  dataset that can fit into a single Kaggle repository. To ensure that these 2,000 samples are representative of the different flows encountered in each configuration, we:

\begin{enumerate}%[leftmargin=*]
    \item Extract four statistical moments of the three velocity components of each of the initial 12,750 sub-volumes. These moments are well-established for characterizing turbulence~\cite{pope2000turbulent}. 
    \item Apply k-means clustering with the elbow method (using the statistical moments as features) to partition the sub-volumes in 18 clusters.
    \item Select 2,000 samples while ensuring that the proportion of clusters are well-balanced.
\end{enumerate}


The resulting sub-volumes form the labels  of  BLASTNet Momentum128 3D SR dataset. \Cref{fig:stats_rhoe} demonstrate the mean and standard deviation of the specific kinetic energy:
\begin{equation}
    \rho e^k = \rho( {u_1}^2+{u_2}^2+{u_3}^2)/2 \, ,
    \label{eq:kin}
\end{equation}
which we use to characterize all channel variables. Each distinct marker represents a different simulation configuration. Since flows from the same configuration possess similar statistics, the different configurations from BLASTNet 2.0 can result in a dataset with a variety of flow conditions.


\DIFdelbegin %DIFDELCMD < \begin{wrapfigure}[19]{r}{0.4\textwidth}
%DIFDELCMD <     \centering
%DIFDELCMD <     %%%
%DIF <  \hspace{-10mm}
    %DIF <  \vspace{-3mm}
%DIFDELCMD < \includegraphics[width=0.4\textwidth]{figs/mean_std_energy_scatter.pdf}
%DIFDELCMD <    %%%
%DIFDELCMD < \caption{%
{%DIFAUXCMD
\DIFdel{To generate the input for turbulent SR, we filter }\DIFdelend \DIFaddbegin \DIFadd{Due to stochastic and chaotic nature of turbulence~\mbox{%DIFAUXCMD
\cite{ottino1990mixing}}\hskip0pt%DIFAUXCMD
, it is not possible to obtain matching pairs of coarse (also known as implicit LES~\mbox{%DIFAUXCMD
\cite{moser2021statistical}}\hskip0pt%DIFAUXCMD
) and fine DNS data. Thus, we employ a canonical method~\mbox{%DIFAUXCMD
\cite{BODE20212617,moser2021statistical,germano1992turbulence} }\hskip0pt%DIFAUXCMD
for obtaining implicit LES surrogates, known as finite-volume optimal LES~\mbox{%DIFAUXCMD
\cite{moser2009}  }\hskip0pt%DIFAUXCMD
(see }\customref{sec:favre} \DIFadd{on their validity). Specifically, we Favre-filter~\mbox{%DIFAUXCMD
\cite{peters_2000} }\hskip0pt%DIFAUXCMD
}\DIFaddend and downsample the labels by 8, 16, and 32$\times$ \DIFdelbegin \DIFdel{. These downsampling ratios are selected based on }\DIFdelend \DIFaddbegin \DIFadd{to obtain }\DIFaddend a representative range of \DIFdelbegin \DIFdel{coarse-grid resolution in LES , which }\DIFdelend \DIFaddbegin \DIFadd{coarse resolution samples (LES }\DIFaddend is typically an order of magnitude coarser than DNS~\cite{pope2000turbulent,griffin_grid}\DIFdelbegin \DIFdel{. Similar to other studies for compressible turbulence, we employ Favre filtering, which involves the following volume-integral~\mbox{%DIFAUXCMD
\cite{peters_2000}}\hskip0pt%DIFAUXCMD
:
}\DIFdelend \DIFaddbegin \DIFadd{) to generate inputs for turbulent SR:
}\DIFaddend \begin{equation}
\label{eq:favre}
    \widetilde{\phi} = \DIFdelbegin \DIFdel{\frac{1}{\ol{\rho}}}\DIFdelend \DIFaddbegin \DIFadd{\frac{1}{\ol{\rho}V_f}}\DIFaddend \int\DIFdelbegin \DIFdel{_V{{\rho \phi}}}\DIFdelend \DIFaddbegin \DIFadd{_{V_f}{{\rho \phi}}}\DIFaddend \,dV\DIFaddbegin \DIFadd{_f
}\DIFaddend \end{equation}
where $\ol{\phi}$ denotes a uniform-filtered  quantity\DIFdelbegin \DIFdel{and }\DIFdelend \DIFaddbegin \DIFadd{, }\DIFaddend $\widetilde{\phi}$ is a Favre-filtered quantity\DIFdelbegin \DIFdel{. Thus, in }\DIFdelend \DIFaddbegin \DIFadd{, and $V_f$ is a subvolume with the size of the filter width. In }\DIFaddend our SR dataset, the channels of each label  correspond to $\phi=\,$\{${\rho}$,${u}_{1}$,${u}_{2}$,${u}_{3}$\}, while the feature channels consist of  $\phi_f=\,$\{$\ol{\rho}$,$\widetilde{u}_{1}$,$\widetilde{u}_{2}$,$\widetilde{u}_{3}$\}. For the purpose of the present benchmark study, we further split the 2000 sub-volumes as follows:


% As mentioned in \Cref{sec:related}, SR of the 3D flows can be useful for a wide-range of applications in turbulence modeling.

% the SR dataset can be  coarse-grid simulations (LES) are typically employed for 
% In the  \textit{a priori} analysis carried out in this study, a top-hat filter $H$ with a desired filter size $\overline{\Delta}$ is applied on a arbitrary quantity $\phi$ from the DNS data through a volume integral:
% \begin{align}
%     \overline{\phi(\mathbf{x})} &= \int_V \phi(\mathbf{x}) H(\mathbf{x} - \mathbf{y},{\Delta_f}) d\mathbf{y}~,\\
%     H(\mathbf{x} - \mathbf{y},{\Delta_f}) &= 
%     \begin{cases}
%         \frac{1}{{\Delta_f}} &  \textrm{for }|\mathbf{x} - \mathbf{y}| \leq {\Delta_f}/2, \\
%         0 & \text{otherwise. }\\
%     \end{cases}
% \end{align}
% and Favre-averaged quantity:





\paragraph{Train, Validation, and Baseline Test Sets} 80:10:10 split via random selection with a uniform distribution. The training set contains 1382 samples, and both validation and baseline test sets contain 173 samples each. %, and baseline test set contains 173.    

\begin{figure}
    \centering
    %DIF >  \vspace{-3mm}
\includegraphics[width=0.37\textwidth]{figs/mean_std_energy_scatter.pdf}
   \caption{ {Statistics of the specific kinetic energy $\rho e^k$ of each 128$^3$ sub-volume in  the  Momentum128 3D SR dataset. Marker type represents DNS configuration. See detailed legend in }\customref{sec:dns_mom} }
    \label{fig:stats_rhoe}
\end{figure}

\paragraph{Parametric Variation Set} A 144-sample subset for model evaluation from an unseen parametric variation configuration with approximately $15\%$ higher mean velocities and velocity fluctuations than the train, validation, and baseline test sets.

\paragraph{Forced HIT Set} A 128-sample subset for model evaluation from an unseen \DIFdelbegin \DIFdel{configuration with 30-fold higher pressure, unseen }\DIFdelend flow type (forced HIT) \DIFdelbegin \DIFdel{, }\DIFdelend \DIFaddbegin \DIFadd{with 30-fold higher pressure }\DIFaddend and 34-fold lower velocity fluctuations.

% Note that in all three evaluation sets, we choose the data that originates from configurations with at least one axis contains  periodic boundary condition. This is done to ensure that Fourier Transforms used in evaluating the turbulent spectra evaluation metric in \Cref{sec:metrics} remains physically valid.  such that at least one axis Further details on the subselection, downsampling, filtering, and split are provided in the \comment{Supplementary Material}.

\section{Benchmark Configuration}
\label{sec:method}
\subsection{Models and Methods}
In this work, three well-studied 2D ResNet-based~\cite{he2016deep} SR models are modified from their original repositories for 3D SR: (i) Residual-in-Residual Dense Block  (RRDB)~\cite{wang2018esrgan}, (ii) Enhanced Deep Residual Super-resolution (EDSR)~\cite{lim2017enhanced}, and  (iii) Residual Channel Attention Networks (RCAN)~\cite{zhang2018image}. \DIFaddbegin \DIFadd{Convolution networks possess inductive biases that are suitable for problems involving spatial grids such as in flow physics~\mbox{%DIFAUXCMD
\cite{Karniadakis2021,kochkov2021machine}}\hskip0pt%DIFAUXCMD
. }\DIFaddend We choose to study these models due to their \DIFdelbegin \DIFdel{difference }\DIFdelend \DIFaddbegin \DIFadd{differences }\DIFaddend in architecture paradigms. Specifically, RRDB employs residual layers within residual layers; EDSR features an expanded network width; RCAN utilizes long skip connections and channel attention mechanisms. \DIFdelbegin \DIFdel{We also }\DIFdelend \DIFaddbegin \DIFadd{In addition, we consider two additional scientific ML approaches: (i) a Conv-FNO model~\mbox{%DIFAUXCMD
\cite{WEN2022104180}}\hskip0pt%DIFAUXCMD
, modified for SR (see details in }\customref{sec:add_model}\DIFadd{), and (ii) an RRDB model regularized with the weighted MSE of the gradient of channel variables $\lambda \Delta^2\sum_{k=1}^{3}\text{MSE}[(\nabla {\hat{\phi}})_{k},(\nabla {{\phi}})_{k}]$~\mbox{%DIFAUXCMD
\cite{yu2022gradient} }\hskip0pt%DIFAUXCMD
to  the loss $(1-\lambda) \text{MSE}(\hat{\phi},{{\phi}})$, where $\Delta$ is the distance between each voxel. Details on the gradient-based loss and its weighting factor $\lambda$ are provided in }\customref{sec:loss}\DIFadd{.
We }\DIFaddend compare model predictions with a baseline approach, \textit{i.e.}, tricubic interpolation. % (performed with \lstinline{scipy.ndimage.zoom}). 
To investigate the scaling behavior of the model architectures, we vary the number of parameters by changing the network depth and width. 

Similar to other turbulent SR studies~\cite{BODE20212617,fukami2019super}, all models are trained with mean-squared-error (MSE) loss, unless otherwise stated. For evaluation, we select models with the best MSE after training for 1,500 epochs with a batch size of 64 across 16 Nvidia V100 GPUs. Learning rate is initialized at \lstinline{1e-4}, and halved every 300 epochs.
Both the number of training iterations and learning scheduling are chosen to match other  SR studies~\cite{wang2018esrgan,lim2017enhanced,zhang2018image} and are found to be sufficient for the SR predictions, as will be shown in \Cref{sec:results}.  All other hyperparameters are maintained from their original studies, with all  models initialized via~\citet{he2015delving}. 
Data augmentation is performed via variants of random rotation and flip -- modified to ensure that augmented data remains consistent with continuity~(\Cref{eq:continuity}).  Training is performed with automatic mixed-precision from \lstinline{Lightning}~\lstinline{1.6.5}~\cite{lightning}. Prior to training, data is normalized with means and standard deviations of density and velocity extracted from the train set.  During evaluation, this normalization resulted in poor accuracy for the Forced HIT set, due to the significantly different magnitudes of density and velocity. However, \Cref{sec:results} will show that good performance can be achieved when normalization is performed with the mean and standard deviation of each distinct evaluation set. Thus, all evaluation sets are normalized with their own mean and standard deviation, prior to testing. All 40 model variations are trained with three different seeds, resulting in a total computational cost of approximately \DIFdelbegin \DIFdel{13}\DIFdelend \DIFaddbegin \DIFadd{15}\DIFaddend ,000~GPU-hours on the Lassen Supercomputer~\cite{patki_lassen2021}. Further information on model hyperparameters, data augmentation, training, normalization, as well as links to code and model weights are found in \customref{sec:url}\DIFdelbegin \DIFdel{, \ref{sec:add_method}, and \ref{sec:add_results}}\DIFdelend \DIFaddbegin \customreftwo{sec:add_method}\customreftwoand{sec:add_results}\DIFaddend .

\subsection{Metrics}
\label{sec:metrics}
We compare the performance of each model by \DIFdelbegin \DIFdel{employing the following metrics based on a }\DIFdelend \DIFaddbegin \DIFadd{examining local and global quantities of each sample. For the local quantities, we employ $\text{Metrics} = \{\text{SSIM},\text{NRMSE}\}$, where SSIM is the }\DIFaddend 3D extension~\cite{ssim3D} of the structural similarity image measure~\DIFdelbegin \DIFdel{(SSIM)~\mbox{%DIFAUXCMD
\cite{wangSSIM} }\hskip0pt%DIFAUXCMD
with $\hat{\phi}$ denoting an arbitrary predicted quantity }\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\cite{wangSSIM} }\hskip0pt%DIFAUXCMD
and NRMSE is the normalized root-mean-squared error }\DIFaddend (see \customref{sec:ssim}\DIFdelbegin \DIFdel{for exact definition and implementation details)}\DIFdelend \DIFaddbegin \DIFadd{). For quantities with multiple channels}\DIFaddend :
\begin{subequations}
    \begin{align}
    \DIFdelbegin \DIFdel{\text{SSIM}}\DIFdelend \DIFaddbegin \DIFadd{\text{Metric}}\DIFaddend _{\rho,\mathbf{u}} &\equiv \frac{1}{4}\left [\DIFdelbegin \DIFdel{\text{SSIM}}\DIFdelend \DIFaddbegin \DIFadd{\text{Metric}}\DIFaddend (\hat{\rho},\rho) + \sum_{i=1}^3 \DIFdelbegin \DIFdel{\text{SSIM}}\DIFdelend \DIFaddbegin \DIFadd{\text{Metric}}\DIFaddend (\hat{u}_i,u_i) \right] \, , \\
    \DIFdelbegin \DIFdel{\text{SSIM}}\DIFdelend \DIFaddbegin \DIFadd{\text{Metric}}\DIFaddend _{sgs} &\equiv \frac{1}{3} \sum_{k=1}^3 \DIFdelbegin \DIFdel{\text{SSIM}[{(\nabla \cdot \hat{\boldsymbol{\tau}}^{\text{sgs}})}_k, (\nabla \cdot \boldsymbol{\tau}^{\text{sgs}})_k] }\DIFdelend \DIFaddbegin \DIFadd{\text{Metric}[{(\nabla \cdot \hat{\boldsymbol{\tau}}^{\text{sgs}})}_k, (\nabla \cdot \boldsymbol{\tau}^{\text{sgs}})_k] }\DIFaddend \, .\label{eq:ssimsgs} 
    % \\
    %     \text{RMSE}_{ E}&=\sqrt{\frac{1}{N_d N_\kappa} \sum_{i=1}^{N_d}\sum_{k=1}^{N_{\kappa}} \left (\log_{10} \frac{E({u}_3)_{k,i}}{E(\hat{u}_3)_{k,i}}\right )^2}\, , 
    \end{align}
\end{subequations}
\DIFdelbegin \DIFdel{$\text{SSIM}_{\rho,\mathbf{u}}$ is similar to  conventional SSIM used in computer vision, where the SSIM of each channel is averaged. Although this metric was originally developed for measuring image similarity, it }\DIFdelend \DIFaddbegin \DIFadd{with $\hat{\phi}$ denoting an arbitrary predicted quantity.
 SSIM is a common image metric, but }\DIFaddend has also become a popular ML metric for evaluating flow simulations \DIFdelbegin \DIFdel{~\mbox{%DIFAUXCMD
\cite{glaws2020}}\hskip0pt%DIFAUXCMD
. We choose  this metric due to its intuitive nature }\DIFdelend \DIFaddbegin \DIFadd{due to its employment of mean, variance, and covariance quantities -- suited for evaluating the statistical nature of turbulence~\mbox{%DIFAUXCMD
\cite{pope2000turbulent,glaws2020,pmlr-v180-bao22a}}\hskip0pt%DIFAUXCMD
. In addition,  this metric can be intuitive }\DIFaddend for both readers familiar and unfamiliar with turbulent flows -- SSIM of 0 denotes dissimilar fields while SSIM of 1 denotes highly similar fields. \DIFdelbegin \DIFdel{Its non-dimensional nature (unlike MSE) also enables physical quantities with different units (}\textit{\DIFdel{e.g.}}%DIFAUXCMD
\DIFdel{, density }%DIFDELCMD < [%%%
\DIFdel{kgm$^{-3}$}%DIFDELCMD < ] %%%
\DIFdel{and velocity }%DIFDELCMD < [%%%
\DIFdel{ms$^{-1}$}%DIFDELCMD < ]%%%
\DIFdel{) to be averaged together}\DIFdelend \DIFaddbegin \DIFadd{$\text{Metric}_{\rho,\mathbf{u}}$ evaluates each channel of the predictions via macro-averaging}\DIFaddend . To measure the suitability of SR for turbulence modeling in coarse-grid simulations, we measure \DIFdelbegin \DIFdel{$\text{SSIM}_{sgs}$}\DIFdelend \DIFaddbegin \DIFadd{$\text{Metric}_{sgs}$}\DIFaddend , which evaluates the predicted divergence of the subgrid-scale \DIFaddbegin \DIFadd{(SGS) }\DIFaddend stress $\nabla \cdot \boldsymbol{\tau}^{\text{sgs}}$. $\nabla \cdot \boldsymbol{\tau}^{\text{sgs}}$ represents physics information lost during coarse-graining, and originates from \DIFdelbegin \DIFdel{Favre-filtering (}%DIFDELCMD < \Cref{eq:favre}%%%
\DIFdel{) the }\DIFdelend \DIFaddbegin \DIFadd{the Favre-filtered/LES  }\DIFaddend momentum equation (\Cref{eq:momentum}):
\begin{align}
    %%%%%% eq2
    &\partial_t (\ol{\rho} \widetilde{\mathbf{u}}) + \nabla \cdot (\ol{\rho} \widetilde{\mathbf{u}}\DIFaddbegin \DIFadd{\otimes }\DIFaddend \widetilde{\mathbf{u}} ) = 
    - \nabla \ol{p}
    + \nabla \cdot( \ol{\boldsymbol{\tau}}+  {\boldsymbol{\tau}}^{\text{sgs}})\, , \quad \text{where} \nonumber \\
    &\tau\DIFdelbegin \DIFdel{_{ij}}\DIFdelend ^{\text{sgs}} = \ol{\rho}(\DIFdelbegin %DIFDELCMD < \widetilde{u_i u_j} %%%
\DIFdelend \DIFaddbegin \widetilde{\mathbf{u} \otimes \mathbf{u}} \DIFaddend - \DIFdelbegin %DIFDELCMD < \widetilde{u}%%%
\DIFdel{_i}%DIFDELCMD < \widetilde{u}%%%
\DIFdel{_j}\DIFdelend \DIFaddbegin \widetilde{\mathbf{u}}\DIFadd{\otimes}\widetilde{\mathbf{u}}\DIFaddend ) \, \DIFdelbegin \DIFdel{, \, i\in }%DIFDELCMD < [%%%
\DIFdel{1,3}%DIFDELCMD < ]%%%
\DIFdel{, j\in }%DIFDELCMD < [%%%
\DIFdel{1,3}%DIFDELCMD < ] %%%
\DIFdel{\, }\DIFdelend .
    \label{eq:sgs} 
\end{align}
\DIFdelbegin %DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdelend \DIFaddbegin \DIFadd{We evaluate global physical properties of ML predictions by considering the NRMSE$_{\{E^k,\varepsilon\}}$ of turbulent dissipation rate $\varepsilon$ (rate of conversion of turbulent kinetic energy to heat) and volume-averaged kinetic energy $E^k$ (momentum component in energy conservation of a fixed control volume): 
}\begin{subequations}
    \begin{align}
    \DIFadd{E^k }&\DIFadd{= \frac{1}{V}\int_V \rho e^k \, dV\, , }\\
    \DIFadd{\varepsilon  }&\DIFadd{=\frac{1}{V} \int_V  \frac{\boldsymbol{\tau}}{\rho} \colon \nabla \mathbf{u} \, dV \, ,
    }\end{align}
\end{subequations}
\DIFadd{with sample volume $V$ and  velocity fluctuation $\mathbf{u}'$.
}\DIFaddend % Here, we propose the 
%  use of RMSE$_E$ for evaluating the quality of turbulence across different scales. RMSE$_E$ represents the root-mean-squared error of the logarithm of the 1D turbulent kinetic energy (TKE) spectra in the $z$-direction. Log-log plots of the TKE spectra is usually employed for evaluating the turbulent properties across different lengthscales/wavenumbers in simulations with periodic domains. Here, we employ evaluate the 1D TKE spectra since all data in the three evaluation sets originate from configurations with periodic boundary conditions in the $z$-direction.



\section{Experiment Results}
\label{sec:results}
We summarize \DIFdelbegin \DIFdel{our evaluation }\DIFdelend \DIFaddbegin \DIFadd{SSIMs }\DIFaddend of RRDB, EDSR, \DIFdelbegin \DIFdel{and RCAN}\DIFdelend \DIFaddbegin \DIFadd{RCAN, and Conv-FNO }\DIFaddend in \Cref{tab:results}, along with model parameters $N_p$ and inferencing cost (in FLOPs \DIFdelbegin \DIFdel{) }\DIFdelend for a batch size of \DIFdelbegin \DIFdel{1.  We also examine an additional RRDB model trained with a popular physics-informed loss term~\mbox{%DIFAUXCMD
\cite{yu2022gradient}}\hskip0pt%DIFAUXCMD
: this is performed by adding the weighted MSE of the gradient of channel variables $\lambda \Delta^2\sum_{k=1}^{3}\text{MSE}[(\nabla {\hat{\phi}})_{k},(\nabla {{\phi}})_{k}]$ to  the loss $(1-\lambda) \text{MSE}(\hat{\phi},{{\phi}})$, where $\Delta$ is the distance between each voxel.   Here, we use the weighting factor $\lambda=0.99$, which was determined from a hyperparameter search as detailed in }%DIFDELCMD < \customref{sec:loss}%%%
\DIFdel{, along with our approach in estimating FLOPs. The  }\DIFdelend \DIFaddbegin \DIFadd{1; see }\customref{sec:flops} \DIFadd{for details).   The  8$\times$ SR }\DIFaddend models shown here possess the best SSIMs across different sizes \DIFdelbegin \DIFdel{investigated at 8$\times$ SR }\DIFdelend for a given model approach, as shown in \customref{sec:all_8x}.  Models \DIFdelbegin \DIFdel{, }\DIFdelend with the same network depth and width, are then initialized and trained for 16 and 32$\times$ SR. 
For 8 and 16$\times$~SR, RRDB (with gradient loss) performs the best across most of the metrics and evaluation sets, with RCAN demonstrating the highest SSIM$_{\rho\text{,}\mathbf{u}}$ at 8$\times$~SR.
At 32$\times$~SR, all shown models exhibit lower  $\text{SSIM}_{\rho,\mathbf{u}}$  than tricubic interpolation in the baseline test set, indicating that SR is difficult to learn at high ratios. However, all models exhibit higher SSIM$_{sgs}$ than tricubic interpolation for all SR ratios. This indicates that SR models may still be useful for turbulence modeling at high SR ratios. \DIFdelbegin \DIFdel{In }\DIFdelend \Cref{fig:upscale}, \DIFdelbegin \DIFdel{we compare the }\DIFdelend \DIFaddbegin \DIFadd{demonstrates that model predictions of }\DIFaddend specific kinetic energy $\rho e^k$ (\Cref{eq:kin}) \DIFdelbegin \DIFdel{, }\DIFdelend \DIFaddbegin \DIFadd{(}\DIFaddend a physical quantity that combines predictions of all four channels\DIFdelbegin \DIFdel{, }\DIFdelend \DIFaddbegin \DIFadd{) }\DIFaddend from all models presented in \Cref{tab:results} \DIFdelbegin \DIFdel{. At 8$\times$ SR, all shown models capture the fine structures of turbulence from the ground truth. This is reflected by the high $\text{SSIM}_{\rho,\mathbf{u}}$ values in }%DIFDELCMD < \Cref{tab:results}%%%
\DIFdel{. As the feature becomes coarser at 16 and 32$\times$ SR,  fine turbulent structures can no longer be recovered}\DIFdelend \DIFaddbegin \DIFadd{increasingly lose fine turbulent structures as SR ratio increase}\DIFaddend . Nevertheless, when compared to tricubic interpolation, the SR models can still recover the magnitudes of the energy at these SR ratios. \DIFdelbegin %DIFDELCMD < \begin{figure} %%%
\DIFdelend \DIFaddbegin \DIFadd{Further examination of the NRMSE metrics from the 8$\times$ SR models (see }\customref{sec:all_8x} \DIFadd{for 16, 32$\times$ SR),  in }\Cref{tab:nrmse}\DIFadd{, also demonstrates that all ML models significantly outperform tricubic interpolation on baseline test and forced HIT sets. Here, gradient loss RRDB performs best in most of the metrics. However, EDSR outperforms with NRMSE$_{E^k}$, as the gradient loss only offers minor improvements to $E^k$. }\DIFaddend


\DIFaddend \begin{table}[!htb]
\DIFdelbeginFL %DIFDELCMD < \vspace{-4mm}
%DIFDELCMD < %%%
\DIFdelendFL \DIFaddbeginFL \vspace{-2mm}
\DIFaddendFL \centering
\DIFdelbeginFL %DIFDELCMD < \fontsize{8.3pt}{8.3pt}%%%
\DIFdelendFL \DIFaddbeginFL \fontsize{8pt}{8.3pt}\DIFaddendFL \selectfont
    \setlength{\tabcolsep}{0.5mm} % General space between cols (6pt standard)
\renewcommand{\arraystretch}{1.1} % 
\caption{Comparison of \DIFdelbeginFL \DIFdelFL{four }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{SSIM of five }\DIFaddendFL models at three SR ratios, with tricubic interpolation. Mean and standard deviation from three  seeds are reported here. \textbf{Bold} term represents best mean.}
\vspace{11pt}
    \label{tab:results}
   \begin{tabular}{lllllllcc}
\toprule
 \multirow{2}{*}{Models} & \multicolumn{2}{c}{{Baseline Test Set}} & \multicolumn{2}{c}{{Param. Variation Set}} & \multicolumn{2}{c}{{ Forced HIT
 Set}}   & \multicolumn{2}{c}{{Size $N_p$ and Cost}} \\
 \cline{2-9}
&  \multicolumn{1}{c}{$\uparrow$SSIM$_{\rho\text{,}\mathbf{u}}$} &   \multicolumn{1}{c}{$\uparrow$SSIM$_{{sgs}}$}  & \multicolumn{1}{c}{$\uparrow$SSIM$_{\rho,\mathbf{u}}$} &   \multicolumn{1}{c}{$\uparrow$SSIM$_{{sgs}}$}  &  \multicolumn{1}{c}{$\uparrow$SSIM$_{\rho\text{,}\mathbf{u}}$} &   \multicolumn{1}{c}{$\uparrow$SSIM$_{{sgs}}$} & $N_p$& $\downarrow$GFLOPs \\
 % & $\uparrow$ & $\uparrow$  & $\uparrow$ & $\uparrow$ & $\uparrow$ & $\uparrow$   & & $\downarrow$ \\
\midrule
 Tricubic 8$\times$ &                    0.820 &                    0.431 &                    0.800 &                    0.418 &                    0.951 &                    0.711 &                    $-$ &           \textbf{22} \\
     RRDB 8$\times$ &          0.907$\pm$0.003 &          0.715$\pm$0.004 &          0.898$\pm$0.003 &          0.755$\pm$0.002 &          0.997$\pm$0.000 &          0.891$\pm$0.003 & \multirow{2}{*}{50.2M} & \multirow{2}{*}{1430} \\
     (+ Grad. Loss) & \textbf{0.936$\pm$0.003} & \textbf{0.802$\pm$0.003} & \textbf{0.929$\pm$0.001} & \textbf{0.825$\pm$0.001} &          0.998$\pm$0.000 & \textbf{0.944$\pm$0.005} &                        &                       \\
     EDSR 8$\times$ &          0.928$\pm$0.004 &          0.748$\pm$0.012 &          0.916$\pm$0.005 &          0.775$\pm$0.010 & {0.999$\pm$0.000} &          0.937$\pm$0.005 &                  34.6M &                  2122 \\
     RCAN 8$\times$ &          0.928$\pm$0.000 &          0.753$\pm$0.002 &          0.916$\pm$0.001 &          0.778$\pm$0.001 & \textbf{0.999$\pm$0.000} &          0.941$\pm$0.003 &                  16.4M &                   671 \\
  \DIFaddbeginFL \DIFaddFL{Conv-FNO 8$\times$ }&          \DIFaddFL{0.846$\pm$0.016 }&          \DIFaddFL{0.566$\pm$0.019 }&          \DIFaddFL{0.845$\pm$0.011 }&          \DIFaddFL{0.614$\pm$0.015 }&          \DIFaddFL{0.993$\pm$0.001 }&          \DIFaddFL{0.845$\pm$0.008 }&                  \DIFaddFL{33.0M }&                  \DIFaddFL{1276 }\\

\midrule
     \DIFaddendFL 
Tricubic 16$\times$ &                    0.652 &                    0.175 &                    0.620 &                    0.173 &                    0.876 &                    0.432 &                    $-$ &           \textbf{22} \\
    RRDB 16$\times$ &          0.724$\pm$0.001 &          0.506$\pm$0.004 &          0.700$\pm$0.001 &          0.512$\pm$0.002 &          0.971$\pm$0.000 &          0.805$\pm$0.003 & \multirow{2}{*}{50.3M} & \multirow{2}{*}{1074} \\
     (+ Grad. Loss) & \textbf{0.739$\pm$0.008} & \textbf{0.554$\pm$0.001} & \textbf{0.719$\pm$0.004} & \textbf{0.556$\pm$0.002} & \textbf{0.973$\pm$0.000} & \textbf{0.816$\pm$0.001} &                        &                       \\
    EDSR 16$\times$ &          0.716$\pm$0.005 &          0.477$\pm$0.018 &          0.693$\pm$0.005 &          0.481$\pm$0.019 &          0.969$\pm$0.001 &          0.783$\pm$0.008 &                  37.8M &                  1944 \\
    RCAN 16$\times$ &          0.672$\pm$0.039 &          0.408$\pm$0.066 &          0.665$\pm$0.024 &          0.415$\pm$0.058 &          0.961$\pm$0.009 &          0.737$\pm$0.050 &                  17.3M &                   573 \\
     \DIFaddbeginFL \DIFaddFL{Conv-FNO 16$\times$ }&          \DIFaddFL{0.629$\pm$0.020 }&          \DIFaddFL{0.343$\pm$0.027 }&          \DIFaddFL{0.640$\pm$0.013 }&          \DIFaddFL{0.355$\pm$0.022 }&          \DIFaddFL{0.951$\pm$0.006 }&          \DIFaddFL{0.690$\pm$0.022 }&                  \DIFaddFL{34.6M }&                  \DIFaddFL{1068 }\\
     \midrule
    \DIFaddendFL
Tricubic 32$\times$ &            \textbf{0.508} &                    0.060 &                    0.476 &                    0.087 &                    0.758 &                    0.156 &                    $-$ &           \textbf{22} \\
    RRDB 32$\times$ &          0.503$\pm$0.001 & \textbf{0.194$\pm$0.005} &          0.482$\pm$0.000 &          0.186$\pm$0.006 &          0.845$\pm$0.001 &          0.494$\pm$0.011 & \multirow{2}{*}{50.4M} & \multirow{2}{*}{1030} \\
     (+ Grad. Loss) &          0.505$\pm$0.001 &          0.184$\pm$0.009 & \textbf{0.483$\pm$0.001} & \textbf{0.188$\pm$0.002} & \textbf{0.850$\pm$0.000} & \textbf{0.516$\pm$0.012} &                        &                       \\
    EDSR 32$\times$ &          0.502$\pm$0.004 &          0.173$\pm$0.006 &          0.481$\pm$0.002 &          0.187$\pm$0.004 &          0.845$\pm$0.001 &          0.463$\pm$0.005 &                  40.9M &                  1921 \\
    RCAN 32$\times$ &          0.473$\pm$0.006 &          0.168$\pm$0.007 &          0.469$\pm$0.002 &          0.185$\pm$0.005 &          0.837$\pm$0.003 &          0.448$\pm$0.012 &                  18.2M &                   561 \\
     \DIFaddbeginFL \DIFaddFL{Conv-FNO 32$\times$ }&          \DIFaddFL{0.476$\pm$0.004 }&          \DIFaddFL{0.155$\pm$0.012 }&          \DIFaddFL{0.470$\pm$0.001 }&          \DIFaddFL{0.178$\pm$0.003 }&          \DIFaddFL{0.842$\pm$0.002 }&          \DIFaddFL{0.435$\pm$0.013 }&                  \DIFaddFL{36.2M }&                  \DIFaddFL{1023 }\\
\bottomrule
\DIFaddendFL 
\end{tabular}
%DIF <  \vspace{-5.5pt}
\end{table}
\begin{figure}[!htb]
\centering
\DIFdelbeginFL %DIFDELCMD < \centering
%DIFDELCMD < %%%
%DIF <  \vspace{-1mm}
%DIFDELCMD < \includegraphics[width=\textwidth]{figs/extrapRe_upscale_all110.pdf}
%DIFDELCMD <   %%%
%DIF <  \vspace{-5mm}
  \DIFdelendFL \DIFaddbeginFL \vspace{-1mm}
\includegraphics[width=\textwidth]{figs/extrapRe_upscale_all_wFNO110.pdf}
  \vspace{-5mm}
  \DIFaddendFL \caption{\DIFdelbeginFL \DIFdelFL{Prediction }\DIFdelendFL \DIFaddbeginFL \label{fig:upscale} \DIFaddFL{Specific kinetic energy $\rho e^k$ prediction }\DIFaddendFL of one sample from the \DIFdelbeginFL \DIFdelFL{Parametric Variation }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{parametric variation }\DIFaddendFL set with models from \Cref{tab:results}. \DIFdelbeginFL %DIFDELCMD < \label{fig:upscale}%%%
\DIFdelendFL \DIFaddbeginFL \DIFaddFL{Prediction errors are shown in }\customref{sec:all_8x}  \DIFaddendFL }
%DIF <  \vspace{0mm}
\end{figure}
\DIFaddbegin
\begin{table}[!htb]
\vspace{-4mm}
\centering
\caption{\DIFaddFL{Comparison of NRMSE of five models at 8$\times$ SR ratio, with tricubic interpolation. Mean and standard deviation from three  seeds are reported here. }\textbf{\DIFaddFL{Bold}} \DIFaddFL{term represents best mean.}\label{tab:nrmse}}
\vspace{11pt}
\fontsize{8pt}{8pt}\selectfont
    \setlength{\tabcolsep}{0.5mm} %DIF >  General space between cols (6pt standard)
\renewcommand{\arraystretch}{1.1} %DIF >  
\begin{tabular}{lllllllll}
\toprule
 & \multicolumn{4}{c}{{Baseline Test Set}}  & \multicolumn{4}{c}{{ Forced HIT
 Set}} \\
 \cline{2-9}
\DIFaddFL{Models }&  \multicolumn{1}{c}{$\downarrow$NRMSE$_{\rho\text{,}\mathbf{u}}$} &   \multicolumn{1}{c}{$\downarrow$NRMSE$_{{sgs}}$}  & 
\multicolumn{1}{c}{$\downarrow$NRMSE$_{{E^k}}$}  &
\multicolumn{1}{c}{$\downarrow$NRMSE$_{{\epsilon}}$}  &    
\multicolumn{1}{c}{$\downarrow$NRMSE$_{\rho\text{,}\mathbf{u}}$} &   \multicolumn{1}{c}{$\downarrow$NRMSE$_{{sgs}}$}  &  
\multicolumn{1}{c}{$\downarrow$NRMSE$_{{ E^k}}$}  &\multicolumn{1}{c}{$\downarrow$NRMSE$_{{\epsilon}}$}\\
& \multicolumn{1}{c}{($\times10^{-2}$)} & \multicolumn{1}{c}{($\times10^{-1}$)} & \multicolumn{1}{c}{($\times10^{-4}$)} &\multicolumn{1}{c}{($\times10^{-1}$)}& \multicolumn{1}{c}{($\times10^{-3}$)} & \multicolumn{1}{c}{($\times10^{-2}$)} & \multicolumn{1}{c}{($\times10^{-6}$)} &\multicolumn{1}{c}{($\times10^{-4}$)}\\
 %DIF >  & $\uparrow$ & $\uparrow$  & $\uparrow$ & $\uparrow$ & $\uparrow$ & $\uparrow$   & & $\downarrow$ \\
\midrule
 \DIFaddFL{Tricubic 8$\times$ }&                   \DIFaddFL{5.1 }&                  \DIFaddFL{7.5 }&                   \DIFaddFL{8.9 }&                  \DIFaddFL{4.3 }&                   \DIFaddFL{8.8 }&                  \DIFaddFL{31.1 }&                     \DIFaddFL{734.5 }&                     \DIFaddFL{451.7 }\\
     \DIFaddFL{RRDB 8$\times$ }&           \DIFaddFL{0.9$\pm$0.0 }&          \DIFaddFL{2.5$\pm$0.0 }&           \DIFaddFL{0.4$\pm$0.1 }&          \DIFaddFL{1.2$\pm$0.0 }&           \DIFaddFL{0.2$\pm$0.0 }&           \DIFaddFL{2.2$\pm$0.1 }&             \DIFaddFL{39.8$\pm$32.5 }&               \DIFaddFL{0.7$\pm$0.3 }\\
     \DIFaddFL{(+ Grad. Loss) }&  \textbf{\DIFaddFL{0.6$\pm$0.0}} & \textbf{\DIFaddFL{1.4$\pm$0.0}} &           \DIFaddFL{0.4$\pm$0.2 }& \textbf{\DIFaddFL{0.5$\pm$0.0}} &  \textbf{\DIFaddFL{0.1$\pm$0.0}} &  \textbf{\DIFaddFL{1.2$\pm$0.2}} &             \DIFaddFL{33.8$\pm$21.4 }&               \DIFaddFL{0.6$\pm$0.2 }\\
     \DIFaddFL{EDSR 8$\times$ }&           \DIFaddFL{0.9$\pm$0.0 }&          \DIFaddFL{2.3$\pm$0.1 }&  \textbf{\DIFaddFL{0.3$\pm$0.1}} &          \DIFaddFL{1.1$\pm$0.1 }&           \DIFaddFL{0.1$\pm$0.0 }&           \DIFaddFL{1.7$\pm$0.2 }&      \textbf{\DIFaddFL{0.6$\pm$0.2}} &      \textbf{\DIFaddFL{0.2$\pm$0.0}} \\
     \DIFaddFL{RCAN 8$\times$ }&           \DIFaddFL{0.9$\pm$0.0 }&          \DIFaddFL{2.3$\pm$0.0 }&           \DIFaddFL{0.3$\pm$0.0 }&          \DIFaddFL{1.1$\pm$0.0 }&           \DIFaddFL{0.1$\pm$0.0 }&           \DIFaddFL{1.4$\pm$0.1 }&               \DIFaddFL{0.6$\pm$0.1 }&               \DIFaddFL{0.2$\pm$0.0 }\\
  \DIFaddFL{Conv-FNO 8$\times$ }&           \DIFaddFL{1.5$\pm$0.1 }&          \DIFaddFL{4.4$\pm$0.2 }&           \DIFaddFL{0.7$\pm$0.2 }&          \DIFaddFL{1.6$\pm$0.1 }&           \DIFaddFL{0.6$\pm$0.1 }&           \DIFaddFL{6.9$\pm$0.7 }&           \DIFaddFL{163.5$\pm$191.5 }&               \DIFaddFL{3.7$\pm$2.2 }\\
\bottomrule
\end{tabular}
\vspace{-5mm}
\end{table} \DIFaddend

\DIFdelbegin \DIFdel{In this work, we also benchmark the scaling behavior of the four model approaches for 8$\times$ SR. 
}\DIFdelend \DIFaddbegin \DIFadd{Scaling behavior of RRDB is shown in }\DIFaddend \Cref{fig:scaling_qual}\DIFaddbegin \DIFadd{, which }\DIFaddend compares  ground truth and input values of $\rho e^k$ (shown in the first column) with  
 $8\times$~SR predictions from tricubic interpolation 
 and variations of RRDB models. \DIFdelbegin \DIFdel{Our discussion is focused on the predictions in the cyan box. }\DIFdelend For the model predictions, the first row visualizes the specific kinetic energy  $\hat{\rho} \hat{e}^k$, while the second row shows the  error $|\epsilon_{\rho e^k}| = |\hat{\rho}\hat{e}^k - \rho e^k|$ normalized by $\rho e^k_{max}$.  \DIFdelbegin \DIFdel{These results show that at }\DIFdelend \DIFaddbegin \DIFadd{Our discussion is focused on the predictions in the cyan box.  At }\DIFaddend $N_p=0.6$M, RRDB is unable to reconstruct  $\rho e^k$ accurately. \DIFdelbegin \DIFdel{At  $N_p = 4.9$M, }\DIFdelend RRDB's prediction is more accurate than tricubic interpolation \DIFaddbegin \DIFadd{at  $N_p = 4.9$M}\DIFaddend , but spurious structures that originate from the coarse grid can be seen. For $N_p = 50.2$M, the model is sufficiently expressive for eliminating the spurious structures from the flow. The addition of the gradient loss term is shown to reduce prediction errors  from RRDB 50.2M. This trend in improvement is also visible in the bottom row, which shows the \DIFdelbegin \DIFdel{of }\DIFdelend mean divergence of \DIFdelbegin \DIFdel{subgrid-scale stresses (defined by }\DIFdelend \DIFaddbegin \DIFadd{SGS stresses (}\DIFaddend \Cref{eq:sgs}). 
\begin{figure}[!htb]
    \centering
\centering
  \vspace{-1mm}
\includegraphics[width=\textwidth]{figs/test_scale_srres93.pdf}
  \caption{{Predictions from various RRDB models, showing gradual improvement in the cyan box. }\label{fig:scaling_qual}}
  \vspace{-5mm}
\end{figure}
 \DIFaddbegin 
\begin{figure}[htb!]
    \centering
\centering
\includegraphics[width=\textwidth]{figs/scaling_models_wFNO.pdf}
  \vspace{-4.5mm}
  \caption{{Scaling behavior of RRDB (with and without gradient-based loss), EDSR, RCAN and Conv-FNO. RRDB, EDSR  and Conv-FNO models continue to scale at large model sizes.  }\label{fig:scaling_quant_models}}
  \vspace{-2mm}
\end{figure}


\DIFaddend %  \begin{wrapfigure}[18]{r}{0.4\textwidth}
%     \centering
%     \vspace{-5mm}
% \includegraphics[width=0.4\textwidth]{figs/test_scale_srres93_tke.pdf}
%    \caption{ 1D turbulent kinetic energy spectra  extracted from the same sample as \Cref{fig:scaling_qual}.}
%     \label{fig:tke}
% \end{wrapfigure}
% These trends can be further quantified by the 1D turbulent kinetic energy (TKE) spectra, a measure that quantifies turbulent behavior at different lengthscales,  shown in \Cref{fig:tke}. The wavenumber $\kappa$ is the inversely proportional to the turbulent lengthscale. Thus, for the input it can be seen that the TKE spectra is truncated for the larger wavenumbers, since the coarse grid shown in \Cref{fig:scaling_qual} does not sufficiently resolve the turbulent structures.  It can be tricubic interpolation does not capture TKE spectra well between [\lstinline{5e3,2e4}], while gradual improvement in predictions are observed with increasing model parameters, which is also seen in \Cref{fig:scaling_qual}.


 Scaling behavior of RRDB (with and without gradient loss), EDSR, \DIFdelbegin \DIFdel{and RCAN}\DIFdelend \DIFaddbegin \DIFadd{RCAN, and Conv-FNO }\DIFaddend models are examined in \Cref{fig:scaling_quant_models}. 
 %A full table with measurements from the parametric variations explored in \Cref{fig:scaling_quant_models} can be found in the \comment{Supplementary Materials}. 
 SSIM$_{sgs}$  scales differently compared to SSIM$_{\rho,\mathbf{u}}$, indicating the importance of evaluating derived physical quantities from model predictions in flow physics applications. For both SSIMs across all evaluation sets, RCAN models demonstrate  better performance than EDSR and vanilla RRDB models for  $N_p <17$M, but performance deteriorates after this model size.
%DIF <  After  $N_p=10$M, performance of 3D RCAN drops. This drop in performance may be due to its much deeper architecture in comparison EDSR and RRDB. \comment{find}. Performance decrease for very deep networks is a common issue, and is usually attributed to issues related to vanishing gradients~\cite{find} \comment{do i need to prove this?}. 
%DIF <  EDSR's trend line falls in between the trend line from RRDB and RCAN. Similar to RRDB, a significant change (although less than in RRDB) in EDSR's performance can be observed at $N_p=2.7$M, and EDSR's performance does not drop significantly after a certain number of parameters. 
The gradient loss term improves RRDB predictions for all  model parameters explored, resulting in SSIM$_{sgs}$ that exceeds RCAN after $N_p=\,$1.4M for the baseline test and Parametric Variation sets. Thus, this loss term is shown to benefit moderately sized models ($N_p=50.2$M) and data (67~GB), which is in contrast to the notion that physics-based losses are mostly helpful for small models and datasets~\cite{Karniadakis2021}. 
 \DIFaddbegin \DIFadd{Conv-FNO  is seen to outperform the baseline tricubic prediction after approximately 20M parameters.  FNO layers are memory-intensive due to high number of dimensions found in the spectral convolution weights (six in total: one for batches, two for channels, and three for Fourier modes). This memory-intensive nature has been acknowledged by FNO's original developers, with attempts to address this remaining an active research pursuit~\mbox{%DIFAUXCMD
\cite{white2023speeding}}\hskip0pt%DIFAUXCMD
.
}\DIFaddend For all models, both SSIMs are found to scale with $\log_{10}N_p$. All \DIFdelbegin \DIFdel{MSE-based }\DIFdelend \DIFaddbegin \DIFadd{ResNet-based }\DIFaddend models share similar slopes in the scaling relationship between SSIM$_{sgs}$ and log$_{10}N_p$ in the test and Parametric Variation set. However, these slopes can differ when evaluated on another flow configuration\DIFdelbegin \DIFdel{, as seen with Forced HIT set. Forced HIT contains flows in more idealized conditions than  in the two other evaluation sets, which results in higher SSIMs when evaluating tricubic interpolation and SR models on these flows. 
  }%DIFDELCMD < \begin{wrapfigure}[21]{r}{0.37\textwidth}
%DIFDELCMD <     %%%
\DIFdelend \DIFaddbegin \DIFadd{. This is seen with the idealized flows in the Forced HIT set, where higher SSIMs from all predictions and baseline are observed. 
  }\DIFaddend

\DIFaddbegin
  \begin{figure}
     \centering
 \vspace{-2mm}
\includegraphics[width=0.35\textwidth]{figs/scaling_flops_wFNO.pdf}
   \caption{ Scaling behavior with  cost.}
    \label{fig:flop}
\end{figure}
\DIFaddend
\Cref{fig:flop} shows the  relationship between SSIM$_{sgs}$ and inference cost (in FLOPs) for the \DIFdelbegin \DIFdel{four }\DIFdelend \DIFaddbegin \DIFadd{five }\DIFaddend model approaches. SSIM$_{sgs}$ for EDSR, RCAN, and RRDB (with gradient loss) models scales with cost in a similar fashion, after approximately 100~GFLOPs. A steeper scaling relationship is observed for \DIFdelbegin \DIFdel{vanilla RRDB in the test set}\DIFdelend \DIFaddbegin \DIFadd{both Conv-FNO and vanilla RRDB}\DIFaddend . Vanilla RRDB models also do not demonstrate a strong linear relationship with log$_{10}$~GFLOPs when tested on the Forced HIT set. %RRDB
% This indicates that certain architectures (such as RRDB) are not suitable for developing small models.  
%For smaller models, \Cref{fig:scaling_quant_models,fig:flop} clearly demonstrate that model architecture design matters. 

 











  





\section{Conclusion}
\label{sec:conc}
In this work, we released BLASTNet 2.0, a public 3D compressible turbulent reacting and non-reacting flow dataset. From this data, we extracted the Momentum128 3D SR dataset, which we employed for benchmarking 3D SR models at 8, 16, and 32$\times$ SR. SR models are shown to score well in SSIM-based metrics and  capture fine turbulent structures at 8$\times$ SR. For the higher SR ratios, these fine structures cannot be captured, but the SR models can still recover the magnitude of large flow structures. 
% At 8$\times$ SR, RCAN possesses high predictive performance at approximately 2- to 3-fold lower cost compared to EDSR and RRDB.  
Through our scaling analysis, we demonstrate that benefits from a gradient-based \DIFdelbegin \DIFdel{physics-informed }\DIFdelend \DIFaddbegin \DIFadd{physics-based }\DIFaddend loss  persist with model scale -- providing empirical evidence that disagrees with the postulated notion that \DIFdelbegin \DIFdel{physics-informed }\DIFdelend \DIFaddbegin \DIFadd{physics-based }\DIFaddend methods are useful mostly in small model scenarios~\cite{Karniadakis2021}. \DIFdelbegin \DIFdel{We observed }\DIFdelend \DIFaddbegin \DIFadd{However, we recognize that this observation is applicable only to one type of physics-based ML technique, and is not necessarily extendable to other physics-based ML approaches. We observe }\DIFaddend that model  performance scales with the logarithm of model parameters, and that the scaling relationship between SSIM$_{sgs}$ and inference cost are similar for RRDB (with gradient loss), EDSR, and RCAN. We also demonstrate that the choice of model architecture can matter significantly, especially when developing small models for real-time scientific computing applications, and that \DIFdelbegin \DIFdel{physics-informed }\DIFdelend \DIFaddbegin \DIFadd{physics-based }\DIFaddend losses can improve \DIFaddbegin \DIFadd{some metrics of }\DIFaddend poorly performing architectures. With this work, we demonstrate that BLASTNet 2.0 can provide a rich resource for evaluating models for scientific and engineering turbulent flows.   

\paragraph{Limitations and Negative Impact}
% As the data in this work comes from numerical simulations, the data is only as good as its model assumptions and numerical schemes. 
While the compressible reacting flow equations (\Cref{eq:dns}) are valid for a wide range of conditions, improvements could be made to chemical modeling. Specifically, skeletal finite-rate mechanisms and mixture-averaged transport used in these reacting flow DNS have been validated for their configurations, but are not as fully-representative of real-world reactions. However, rectifying this would require detailed mechanisms (introducing an order of magnitude more PDEs) and multi-component transport that can result in intractable calculations~\cite{LU2009192}. Another limitation is that the DNS data originate from proprietary-licensed numerical solvers \DIFdelbegin \DIFdel{. Thus, while these data  have been  validated for published research, the data }\DIFdelend \DIFaddbegin \DIFadd{(see }\customref{sec:dns_config}\DIFadd{), resulting in  data  that }\DIFaddend cannot be thoroughly inspected through open-source means. However, \DIFdelbegin \DIFdel{we note that the }\DIFdelend expertise, peer review \DIFaddbegin \DIFadd{from published research}\DIFaddend , and solver reputation ensure that these DNS data meet community-accepted standards. \DIFdelbegin \DIFdel{We note that generating these data incur }\DIFdelend \DIFaddbegin \DIFadd{In this work, we are limited to using Favre-filtered (}\Cref{eq:favre}\DIFadd{) DNS to generate low-resolution inputs in the Momentum128 3D SR dataset, as it is not feasible to obtain pairs of coarse simulation sample that matches a corresponding ground truth DNS sample, as the chaotic nature of turbulence will result in uncorrelated pairs~\mbox{%DIFAUXCMD
\cite{ottino1990mixing}}\hskip0pt%DIFAUXCMD
. However, Favre-filtered DNS is a canonical surrogate~\mbox{%DIFAUXCMD
\cite{moser2009} }\hskip0pt%DIFAUXCMD
for coarse simulations with strong theoretical foundations~\mbox{%DIFAUXCMD
\cite{germano1992turbulence,moser2021statistical}}\hskip0pt%DIFAUXCMD
. Further discussion on the validity of employing Favre-filtered DNS is provided in }\customref{sec:favre}\DIFadd{.
Data generation incurs }\DIFaddend up to $\mathcal{O}(10^6)$ CPU-hours per case, while this study used \DIFdelbegin \DIFdel{13}\DIFdelend \DIFaddbegin \DIFadd{15}\DIFaddend ,000 GPU-hours -- resulting in significant carbon emissions. However, we  \DIFdelbegin \DIFdel{have }\DIFdelend attempted to ameliorate this by curating previously unreleased already-generated DNS from existing publications, and employing mixed-precision training for this study. In addition, this work can \DIFdelbegin \DIFdel{be used to }\DIFdelend improve fundamental knowledge on carbon-free combustion, which can reduce society-wide reliance on hydrocarbons.
\begin{ack}
The authors acknowledge financial support and computing resources from the U.S. Department of Energy National Nuclear Security Administration, under award No. DE-NA0003968. We also thank the NASA Early Stage Innovation Program with award No. 80NSSC22K0257, and the Department of Energy Office of Energy Efficiency Renewable Energy (EERE) with award No. DE-EE0008875 for funding this work. Wai Tong Chung is grateful for partial financial support from the
Stanford Institute for Human-centered Artificial Intelligence Graduate Fellowship. This research used resources of the National Energy Research Scientific Computing Center (NERSC), a U.S. Department of Energy Office of Science User Facility located at Lawrence Berkeley National Laboratory, operated under Contract No. DE-AC02-05CH11231 using NERSC award ERCAP0021046. We are also grateful to members of the Kaggle staff for fruitful discussions that have contributed to this work. 
\end{ack}

%bib
\bibliographystyle{my_nat.bst}
\bibliography{2_refs.bib}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{We introduce our dataset, describe the benchmark study, and present our conclusions.}
  \item Did you describe the limitations of your work?
    \answerYes{This is done in \Cref{sec:conc}.} 
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{This is also done in \Cref{sec:conc}.} 
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{Our work does not involve human participants. Our data is licensed and consented, while adhering to FAIR~\cite{Wilkinson2016} principles. Attempts to mitigate negative social impacts have been made. }
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{This study involves an empirical benchmark approach. }
	\item Did you include complete proofs of all theoretical results?
    \answerNA{This study involves an empirical benchmark approach.}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{All data is shared via Kaggle and centralized at \url{https://blastnet.github.io}, as mentioned in the abstract and \Cref{sec:blastnet_data}. In addition, links to the code and model weights are shared in \customref{sec:url}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{A summary of training details is provided in \Cref{sec:method}, with data split detailed in \Cref{sec:mom_data}. Further details are also provided in \customref{sec:add_method}.  }
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{All experiments are performed with three different seeds. \Cref{tab:results} shows mean and standard deviations from these runs. \Cref{fig:scaling_quant_models,fig:flop} includes points from all three seeds, with shaded regions demonstrating the standard deviation.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{\Cref{sec:method} mentions that we utilized approximately 13,000 GPU-hours on 16 V100 GPUs on the Lassen supercomputer~\cite{patki_lassen2021}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{All previous studies and solvers used for this study have been cited in \Cref{sec:blastnet_data}. Additionally, assets for training and evaluation are cited in \Cref{sec:method}.}
  \item Did you mention the license of the assets?
    \answerYes{The previously unreleased data is licensed via CC~BY-NC-SA~4.0, as mentioned in \Cref{sec:blastnet_data}.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{All data is shared via Kaggle and centralized at \url{https://blastnet.github.io}, as mentioned in the abstract and \Cref{sec:blastnet_data}. Links to code for this benchmark study is shared in \customref{sec:url}.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{As mentioned in \Cref{sec:blastnet_data}, all published data originate from the present authors.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{Our data has no offensive content. For personally identifiable information, it only contains name and institution of data contributors. This is discussed in \Cref{sec:blastnet_data}.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{No human subjects employed.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{No human subjects employed.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{No human subjects employed.}
\end{enumerate}

\end{enumerate}
